A Fox-Milnor theorem for the Alexander polynomial of knotted $2$-spheres in $S^4$

For knots in $S^3$, it is well-known that the Alexander polynomial of a ribbon knot factorizes as $f(t)f(t^{-1})$ for some polynomial $f(t)$. By contrast, the Alexander polynomial of a ribbon $2$-knot is not even symmetric in general. Via an alternative notion of ribbon $2$-knots, we give a topological condition on a $2$-knot that implies the factorization of the Alexander polynomial.

==> biblio.tex <==
@inproceedings{Artin,
  title={Zur Isotopie zweidimensionaler Fl{\"a}chen imR 4},
  author={Artin, Emil},
  booktitle={Abhandlungen aus dem Mathematischen Seminar der Universit{\"a}t Hamburg},
  volume={4},
  number={1},
  pages={174--177},
  year={1925},
  organization={Springer}
}

@article {Flo,
    AUTHOR = {Florens, V.},
     TITLE = {On the {F}ox-{M}ilnor theorem for the {A}lexander polynomial
              of links},
   JOURNAL = {International Mathematics Research Notices},
      YEAR = {2004},
    NUMBER = {2},
     PAGES = {55--67},
}

@incollection {Fox,
    AUTHOR = {Fox, R. H.},
     TITLE = {Some problems in knot theory},
 BOOKTITLE = {Topology of 3-manifolds and related topics ({P}roc. {T}he
              {U}niv. of {G}eorgia {I}nstitute, 1961)},
     PAGES = {168--176},
 PUBLISHER = {Prentice-Hall, Englewood Cliffs, N.J.},
      YEAR = {1962},
}

@article {FoxMilnor,
    AUTHOR = {Fox, Ralph H. and Milnor, John W.},
     TITLE = {Singularities of {$2$}-spheres in {$4$}-space and cobordism of
              knots},
   JOURNAL = {Osaka Journal of Mathematics},
    VOLUME = {3},
      YEAR = {1966},
     PAGES = {257--267},
}

@article {Gu,
    AUTHOR = {Guti\'errez, M. A.},
     TITLE = {On knot modules},
   JOURNAL = {Inventiones Mathematicae},
    VOLUME = {17},
      YEAR = {1972},
     PAGES = {329--335},
}

@article {Hitt,
    AUTHOR = {Hitt, L. R.},
     TITLE = {Examples of higher-dimensional slice knots which are not
              ribbon knots},
   JOURNAL = {Proceedings of the American Mathematical Society},
    VOLUME = {77},
      YEAR = {1979},
    NUMBER = {2},
     PAGES = {291--297},
}

@Phdthesis{ Hitphd,
  author       = "Hitt, L. R.", 
  title        = "{Handlebody presentations of knot cobordisms}",
  school       = "Florida State University",
  year         = "1977",
  type         = "{Ph.D. Thesis}"
}

@article {Kaw,
    AUTHOR = {Kawauchi, Akio},
     TITLE = {On pseudo-ribbon surface-links},
   JOURNAL = {Journal of Knot Theory and its Ramifications},
    VOLUME = {11},
      YEAR = {2002},
    NUMBER = {7},
     PAGES = {1043--1062},
}

@article {Ker,
    AUTHOR = {Kervaire, Michel A.},
     TITLE = {Les n\oe uds de dimensions sup\'erieures},
   JOURNAL = {Bulletin de la Soci\'et\'e Math\'ematique de France},
    VOLUME = {93},
      YEAR = {1965},
     PAGES = {225--271},
}

@article { Kin,
    AUTHOR = {Kinoshita, Shin'ichi},
     TITLE = {On the {A}lexander polynomials of {$2$}-spheres in a {$4$}--sphere},
   JOURNAL = {Annals of Mathematics (2)},
    VOLUME = {74},
      YEAR = {1961},
     PAGES = {518--531}
}

@article {L1,
    AUTHOR = {Levine, J.},
     TITLE = {Polynomial invariants of knots of codimension two},
   JOURNAL = {Annals of Mathematics (2)},
    VOLUME = {84},
      YEAR = {1966},
     PAGES = {537--554},
}

@article {L2,
    AUTHOR = {Levine, J.},
     TITLE = {Knot cobordism groups in codimension two},
   JOURNAL = {Commentarii Mathematici Helvetici},
    VOLUME = {44},
      YEAR = {1969},
     PAGES = {229--244},
}

@article {L3,
    AUTHOR = {Levine, Jerome},
     TITLE = {Knot modules. {I}},
   JOURNAL = {Transactions of the American Mathematical Society},
    VOLUME = {229},
      YEAR = {1977},
     PAGES = {1--50},
}

@article {L4,
    AUTHOR = {Levine, J.},
     TITLE = {Invariants of knot cobordism},
   JOURNAL = {Inventiones Mathematicae},
    VOLUME = {8},
      YEAR = {1969},
     PAGES = {355},
}

@article {L5,
    AUTHOR = {Levine, J.},
     TITLE = {Unknotting spheres in codimension two},
   JOURNAL = {Topology},
    VOLUME = {4},
      YEAR = {1965},
     PAGES = {9--16},
}

@Article{ M3,
	author = "Delphine Moussard",
	title = "{Rational Blanchfield forms, S-equivalence, and null LP-surgeries}",
	journal = "{Bulletin de la Soci\'et\'e Math\'ematique de France}",
	volume = "143",
	number = "2",
	pages = "403--431",
	year = "2015"
}

@article {NN,
    AUTHOR = {Nakanishi, Yasutaka and Nishizawa, Kazuo},
     TITLE = {On two dimensional knots with reciprocal polynomials},
   JOURNAL = {Journal of Knot Theory and its Ramifications},
    VOLUME = {10},
      YEAR = {2001},
    NUMBER = {6},
     PAGES = {841--850},
}

@article {Sekine,
    AUTHOR = {Fox, Ralph H. and Milnor, John W.},
     TITLE = {Singularities of {$2$}-spheres in {$4$}-space and cobordism of
              knots},
   JOURNAL = {Osaka Journal of Mathematics},
    VOLUME = {3},
      YEAR = {1966},
     PAGES = {257--267},
}

@article{ ShSu,
  title={Homology invariants of cyclic coverings with application to links},
  author={Shinohara, Y and Sumners, DW},
  journal={Transactions of the American Mathematical Society},
  volume={163},
  pages={101--121},
  year={1972}
}

@article { Yan,
    AUTHOR = {Yanagawa, Takaaki},
     TITLE = {On ribbon {$2$}-knots. {T}he {$3$}-manifold bounded by the
              {$2$}-knots},
   JOURNAL = {Osaka J. Math.},
  FJOURNAL = {Osaka Journal of Mathematics},
    VOLUME = {6},
      YEAR = {1969},
     PAGES = {447--464}
}

